Friedrichs' systems discretized with the Discontinuous Galerkin method: domain decomposable model order reduction and Graph Neural Networks approximating vanishing viscosity solutions

Friedrichs' systems (FS) are symmetric positive linear systems of first-order partial differential equations (PDEs), which provide a unified framework for describing various elliptic, parabolic and hyperbolic semi-linear PDEs such as the linearized Euler equations of gas dynamics, the equations of compressible linear elasticity and the Dirac-Klein-Gordon system. FS were studied to approximate PDEs of mixed elliptic and hyperbolic type in the same domain. For this and other reasons, the versatility of the discontinuous Galerkin method (DGM) represents the best approximation space for FS. We implement a distributed memory solver for stationary FS in deal.II. Our focus is model order reduction. Since FS model hyperbolic PDEs, they often suffer from a slow Kolmogorov n-width decay. We develop two approaches to tackle this problem. The first is domain decomposable reduced-order models (DD-ROMs). We will show that the DGM offers a natural formulation of DD-ROMs, in particular regarding interface penalties, compared to the continuous finite element method. We also develop new repartitioning strategies to obtain more efficient local approximations of the solution manifold. The second approach involves graph neural networks used to infer the limit of a succession of projection-based linear ROMs corresponding to lower viscosity constants: the heuristic behind is to develop a multi-fidelity super-resolution paradigm to mimic the mathematical convergence to vanishing viscosity solutions while exploiting to the most interpretable and certified projection-based ROMs.

==> sections/results.tex <==
\subsection{Advection diffusion reaction}
We consider the parametric semi-linear advection diffusion reaction rewritten in mixed form:
\begin{equation}
    \left(
    \begin{array}{c}
        \mu_1^{-1}\boldsymbol{\sigma}(\x) + \nabla u(\x)\\
        \nabla\cdot\boldsymbol{\sigma}(\x) +\mu_2\boldsymbol{\beta}(\x)\cdot\nabla u(\x) + \mu_3 u(\x)
    \end{array}
    \right)
    = 
    \left(
    \begin{array}{c}
        0 \\
        f(\x)
    \end{array}
    \right),
    \quad \forall\x\in\Omega=[-\frac{1}{2}, 2]\times[-1, 1],
\end{equation}
where $(\mu_1, \mu_2, \mu_3)\in\mathbb{R}^3$ the advection velocity $\boldsymbol{\beta}$ and the source term $f$ are defined as follows:
\begin{equation}
    \boldsymbol{\beta}(\x)_1 = 1,
    \qquad
    \boldsymbol{\beta}(\x)_2 =
    \begin{cases}
        0 & x < 0, \\
        \frac{1}{5}x^2\cos{2x^2} + 10^{-1}\sin{2x^2} & x \geq 0.
    \end{cases},
    \quad
    f(\x) = \exp{-\frac{10^{-2}}{\frac{1}{4}^2-\lVert\x\rVert^2}}.
\end{equation}
Mind that $\frac{d}{dx}\left(10^{-1}x\sin{2x^2}\right)= \frac{1}{5}x^2\cos{2x^2} + 10^{-1}\sin{2x^2}$.
A sketch of the domain $\Omega$ with the source term support and the curve that defines the advection field is shown:
\begin{figure}[h]
    \centering
    \includegraphics[width=0.6\textwidth]{figures/ADRDomain.png}
\end{figure}

Homogeneous neumann boundary conditions are applied to the boundary $\partial\Omega$ with the boundary operator
\begin{equation}
    \mathcal{M}=\left[
    \begin{array}{c;{2pt/2pt}c}
        0 & n \\ \hdashline[2pt/2pt]
        -n^t & 0 
    \end{array}\right]
\end{equation}

\subsection{Compressibile linear elasticity}
We consider the parametric compressible linear elasticity system with domain a cylindrical shell along the z-axis with inner radious $1$, outer radious $3$ and height $10$:
\begin{equation}
    \left(
    \begin{array}{c}
        \boldsymbol{\sigma} - \mu_1(\nabla\cdot \ub)\mathbb{I}_3 -2\mu_2\frac{\left(\nabla \ub + (\nabla \ub)^t\right)}{2}\\
        -\frac{1}{2}\nabla\cdot\left(\boldsymbol{\sigma}+\boldsymbol{\sigma}^t\right) +\mu_3 \ub
    \end{array}
    \right)
    = 
    \left(
    \begin{array}{c}
        0 \\
        \mathbf{f}
    \end{array}
    \right),
    \quad \forall\x\in\Omega,
\end{equation}
where $(\mu_1, \mu_2, \mu_3)\in\mathbb{R}^3$ and $\mathbf{f} = (0, -1, 0)$. The system can be rewritten as FS:
\begin{equation}
    \left(
    \begin{array}{c}
        \boldsymbol{\sigma} - \frac{\mu_1}{2\mu_2+3\mu_1}\text{tr}(\boldsymbol{\sigma})\mathbb{I}_3 -\frac{\left(\nabla \ub + (\nabla \ub)^t\right)}{2}\\
        -\frac{1}{2}\nabla\cdot\left(\boldsymbol{\sigma}+\boldsymbol{\sigma}^t\right) +\frac{\mu_3}{2\mu_2} \ub
    \end{array}
    \right)
    = 
    \left(
    \begin{array}{c}
        0 \\
        \mathbf{f}
    \end{array}
    \right),
    \quad \forall\x\in\Omega.
\end{equation}
We show the domain $\Omega$:
\begin{figure}[h]
    \centering
    \includegraphics[width=1\textwidth]{figures/elasticityDomain.png}
\end{figure}

We define the boundaries
\begin{equation}
    \Gamma_D = \partial\Omega\cap\{z=0\}\qquad \Gamma_N = \partial\Omega\setminus \Gamma_D
\end{equation}

Mixed boundary conditions are applied with the boundary operator:
\begin{equation}
    \langle \mathcal{M}(\boldsymbol{\sigma}, u), (\boldsymbol{\tau}, v)\rangle_{V^{'}, V} = 
    \langle \boldsymbol{\sigma}\cdot \n, v\rangle_{-\frac{1}{2}, \frac{1}{2}, \Gamma_D}
    - \langle \boldsymbol{\tau}\cdot \n, u\rangle_{-\frac{1}{2}, \frac{1}{2}, \Gamma_D}
    -\langle \boldsymbol{\sigma}\cdot \n, v\rangle_{-\frac{1}{2}, \frac{1}{2}, \Gamma_N}
    + \langle \boldsymbol{\tau}\cdot \n, u\rangle_{-\frac{1}{2}, \frac{1}{2}, \Gamma_N}
\end{equation}

\subsection{Maxwell equations in stationary regime}
We consider the parametrix Maxwell equations in the stationary regime on a torus $\Omega$, with inner radius $r=0.5$ and outer radius $R=2$:
\begin{equation}
    \left(
    \begin{array}{c}
        \mu\Hb+\nabla\times \Eb\\
        \sigma\Eb-\nabla\times \Hb
    \end{array}
    \right)
    = 
    \left(
    \begin{array}{c}
        \mathbf{g} \\
        \mathbf{f}
    \end{array}
    \right),
    \quad \forall\x\in\Omega,
\end{equation}
the boundary conditions $n\times\Eb = \mathbf{0}$ are applied with the boundary operator
\begin{equation}
    \mathcal{M}=\left[
    \begin{array}{c;{2pt/2pt}c}
        0 & \mathcal{T} \\ \hdashline[2pt/2pt]
        \mathcal{T}^t & 0 
    \end{array}\right]
\end{equation}
where $\mathcal{T}\in\mathbb{R}^{3,3}$ is such that
\begin{equation}
    \mathcal{T}\xi = n\times\xi,\quad\forall\xi\in\mathbb{R}^3.
\end{equation}

We consider the exact solutions
\small
\begin{align*}
    &H_{\text{exact}}(\x)=-\frac{1}{\mu}\left(\frac{2xy}{\sqrt{x^2+z^2}}, \frac{-4y^2\sqrt{x^2+z^2}+\sqrt{x^2+z^2}(-12(x^2+z^2)-15)+32(x^2+z^2)}{4(x^2+z^2)}, \frac{2xy}{\sqrt{x^2+z^2}}\right), \\
    &E_{\text{exact}}(\x)=\left(\frac{z}{\sqrt{x^2+z^2}}, 0, -\frac{x}{\sqrt{x^2+z^2}}\right)\cdot\left(r^2-y^2-\left(R-\sqrt{x^2+z^2}\right)^2\right),
\end{align*}
\normalsize
The source terms are defined consequently as
\begin{equation}
    g(\x)=0,\qquad f(\x)=\sigma E_{\text{exact}}-\nabla\times H_{\text{exact}}.
\end{equation}

We show a solution for $\mu=\sigma=1$:
\begin{figure}[h]
    \centering
    \includegraphics[width=1\textwidth]{figures/maxwellFOM.png}
    \caption{Electric and magnetic fields of the Maxwell equations in stationary regime with Dirichlet homogeneous boundary conditions $\mathbf{n}\times\mathbf{E}=\mathbf{0}$. The vectors of the magnetic and electric fields are scaled by $0.5$ and $2$ of their magnitude respectively.}
\end{figure}
